Online Robust Control of Nonlinear Systems with Large Uncertainty

Robust control is a core approach for controlling systems with performance guarantees that are robust to modeling error, and is widely used in real-world systems. However, current robust control approaches can only handle small system uncertainty, and thus require significant effort in system identification prior to controller design. We present an online approach that robustly controls a nonlinear system under large model uncertainty. Our approach is based on decomposing the problem into two sub-problems, "robust control design" (which assumes small model uncertainty) and "chasing consistent models", which can be solved using existing tools from control theory and online learning, respectively. We provide a learning convergence analysis that yields a finite mistake bound on the number of times performance requirements are not met and can provide strong safety guarantees, by bounding the worst-case state deviation. To the best of our knowledge, this is the first approach for online robust control of nonlinear systems with such learning theoretic and safety guarantees. We also show how to instantiate this framework for general robotic systems, demonstrating the practicality of our approach.

==> binaryseqtikz.tex <==
\usetikzlibrary{chains,fit,shapes}
\usetikzlibrary{decorations.pathreplacing}
\begin{tikzpicture}
\definecolor{blowup}{HTML}{FF511C}
\def \light{ 50 }
\def \dark{ 50 }

\tikzstyle{every path}=[very thick]
\tikzstyle{overbrace text style}=[font=\small, above, pos=.5, yshift=3mm]
\tikzstyle{overbrace style}=[decorate,decoration={brace,raise=1mm,amplitude=4pt},color=blowup!\dark!black]
\tikzstyle{underbrace style}=[decorate,decoration={brace,raise=2mm,amplitude=3pt,mirror},color=gray]
\tikzstyle{underbrace text style}=[font=\small, below, pos=.5, yshift=-3mm]

\edef\sizetape{0.9cm}
\tikzstyle{tmtape}=[draw,minimum size=\sizetape]
\tikzstyle{tmhead}=[arrow box,draw,minimum size=.5cm,arrow box
arrows={east:.25cm, west:0.25cm}]

%% Draw TM tape
\begin{scope}[start chain=1 going right,node distance=-0.15mm]
    \node [on chain=1,tmtape,draw=none](axinput) {\phantom{cost}};
    \node [on chain=1,tmtape, fill = blowup!\light](ta) {1};
    \node [on chain=1,tmtape, fill = blowup!\light] (tb) {1};
    \node [on chain=1,tmtape](tc) {0};
    \node [on chain=1,tmtape, fill = blowup!\light](td) {1};
    \node [on chain=1,tmtape](te) {0};
    \node [on chain=1,tmtape, fill = blowup!\light](tf) {1};
    \node [on chain=1,tmtape, fill = blowup!\light](tg) {1};
    \node [on chain=1,tmtape, fill = blowup!\light](th) {1};
    \node [on chain=1,tmtape](ti) {0};
    \node [on chain=1,tmtape](tj) {0};
    \node [on chain=1,tmtape, fill = blowup!\light](tk) {1};
    \node [on chain=1,tmtape,draw=none](tl) {$\ldots$};
    \node [on chain=1](to) {\textbf{cost} $\cl{G}_t(x_t,u_t)$};
\end{scope}

%% Draw TM Finite Control
% \begin{scope}
% [shift={(3cm,-5cm)},start chain=circle placed {at=(-\tikzchaincount*60:1.5)}]
% \foreach \i in {q_0,q_1,q_2,q_3,\ddots,q_n}
% 	\node [on chain] {$\i$};

% % Arrow to current state
% \node (center) {};
% \draw[->] (center) -- (circle-2);

% \node[rounded corners,draw=black,thick,fit=(circle-1) (circle-2) (circle-3) 
%       (circle-4) (circle-5) (circle-6),
% 			label=below:\textbf{Finite Control}] (fsbox)
% 		{};
% \end{scope}

%% Draw TM head below (input) tape cell
%\node [tmhead,yshift=-.3cm] at (input.south) (head) {$q_1$};
\node [yshift=-.3cm] at (ta.south) {$0$};
\node [yshift=-.3cm] at (tb.south) {$1$};
\node [yshift=-.3cm] at (tc.south) {$2$};
\node [yshift=-.3cm] at (td.south) {$3$};
\node [yshift=-.3cm] at (te.south) {$4$};
\node [yshift=-.3cm] at (tf.south) {$5$};
\node [yshift=-.3cm] at (tg.south) {$6$};
\node [yshift=-.3cm] at (th.south) {$7$};
\node [yshift=-.3cm] at (ti.south) {$8$};
\node [yshift=-.3cm] at (tj.south) {$9$};
\node [yshift=-.3cm] at (tk.south) {$10$};
\node [yshift=-.3cm] at (tl.south) {$\ldots$};
\node [yshift=-.3cm] at (to.south) {};
\node [xshift=-1cm,yshift=-.3cm] at (ta.south west) (head) {\textbf{time} $t$};

\draw [overbrace style] (ta.north west) -- (tb.north east) node [overbrace text style] {$\oneset_1=\{0,1\}$};
\draw [overbrace style] (td.north west) -- (td.north east) node [overbrace text style] {$\oneset_2=\{3\}$};
\draw [overbrace style] (tf.north west) -- (th.north east) node [overbrace text style] {$\oneset_4=\{5,6,7\}$};
\draw [overbrace style] (tk.north west) -- (tl.north east) node [overbrace text style] {$\oneset_5=\{10,\dots\}$};
%% Link Finite Control with Head
% \path[->,draw] (fsbox.north) .. controls (4.5,-1) and (0,-2) .. node[right] 
% 			(headlinetext)
%  			{} 
% 			(head.south);
% \node[xshift=3cm] at (headlinetext)  
% 			{\begin{tabular}{c} 
% 				\textbf{Reading and Writing Head} \\  
% 				\textbf{(moves in both directions)} 
% 			 \end{tabular}};

\end{tikzpicture}

